Pixel-wise Agricultural Image Time Series Classification: Comparisons and a Deformable Prototype-based Approach

Improvements in Earth observation by satellites allow for imagery of ever higher temporal and spatial resolution. Leveraging this data for agricultural monitoring is key for addressing environmental and economic challenges. Current methods for crop segmentation using temporal data either rely on annotated data or are heavily engineered to compensate the lack of supervision. In this paper, we present and compare datasets and methods for both supervised and unsupervised pixel-wise segmentation of satellite image time series (SITS). We also introduce an approach to add invariance to spectral deformations and temporal shifts to classical prototype-based methods such as K-means and Nearest Centroid Classifier (NCC). We study different levels of supervision and show this simple and highly interpretable method achieves the best performance in the low data regime and significantly improves the state of the art for unsupervised classification of agricultural time series on four recent SITS datasets.

==> text/07_acknowledgments.tex <==
\subsubsection*{Acknowledgments}

The work of MA was partly supported by the European Research Council (ERC project DISCOVER, number 101076028). JP was supported in part by the Louis Vuitton/ENS chair on artificial intelligence and the French government under management of Agence Nationale de la Recherche as part of the \textit{Investissements d’avenir} program, reference ANR19-P3IA0001 (PRAIRIE 3IA Institute). This work was granted access to the HPC resources of IDRIS under the allocation 2021-AD011013067 made by GENCI. We thank Antoine Guédon for inspiring discussions; Tom Monnier, Romain Loiseau, Ricardo Garcia Pinel, Théo Bodrito, Yannis Siglidis and Loïc Landrieu for manuscript feedback and constructive insights.
